Practical Benefits of Feature Feedback Under Distribution Shift

In attempts to develop sample-efficient and interpretable algorithms, researcher have explored myriad mechanisms for collecting and exploiting feature feedback (or rationales) auxiliary annotations provided for training (but not test) instances that highlight salient evidence. Examples include bounding boxes around objects and salient spans in text. Despite its intuitive appeal, feature feedback has not delivered significant gains in practical problems as assessed on iid holdout sets. However, recent works on counterfactually augmented data suggest an alternative benefit of supplemental annotations, beyond interpretability: lessening sensitivity to spurious patterns and consequently delivering gains in out-of-domain evaluations. We speculate that while existing methods for incorporating feature feedback have delivered negligible in-sample performance gains, they may nevertheless provide out-of-domain benefits. Our experiments addressing sentiment analysis, show that feature feedback methods perform significantly better on various natural out-of-domain datasets despite comparable in-domain evaluations. By contrast, performance on natural language inference remains comparable. Finally, we compare those tasks where feature feedback does (and does not) help.

==> tables.tex <==
\begin{table}[t!]
\centering
    \small
\begin{tabular}{l c c c}
\toprule
Test set &  Classify-only & \citeauthor{pruthi2020weakly}  & \citeauthor{jain2020learning}\\
\midrule
\multicolumn{4}{c}{BERT}\\
\midrule
In-domain & $85.9_{0.7}$ & $\mathbf{89.9_{2.3}}$ & $\mathbf{90.4_{0.3}}$\\
CRD & $89.3_{0.7}$ & $\mathbf{91.6_{0.7}}$ & $87.5_{0.8}$\\
SST2 & $77.6_{4.1}$ & $79.3_{3.6}$ & $75.6_{1.2}$\\
Amazon & $78.1_{4.9}$ & $83.5_{3.1}$ & $\mathbf{92.3_{1.2}}$\\
Semeval & $70.6_{5.7}$ & $73.2_{2.6}$ & $68.6_{2.2}$\\
Yelp & $86.8_{1.7}$ & $85.7_{1.6}$ & $\mathbf{91.6_{0.1}}$\\ 
\midrule
\multicolumn{4}{c}{ELECTRA}\\
\midrule
In-domain & $93.2_{0.3}$ & $91.8_{1.4}$ & $93.1_{0.3}$\\
CRD & $91.6_{0.4}$ & $\mathbf{93.7_{0.9}}$ & $91.5_{0.7}$\\
SST2 & $73.2_{1.3}$ & $74.0_{1.2}$ & $\mathbf{77.2_{1.4}}$\\
Amazon & $72.8_{2.0}$ & $75.5_{2.1}$ & $\mathbf{84.2_{1.6}}$\\
Semeval & $67.5_{4.5}$ & $72.5_{1.8}$ & $66.7_{3.0}$\\
Yelp & $79.0_{3.6}$ & $\mathbf{84.6_{1.8}}$ & $\mathbf{94.7_{0.2}}$\\
\bottomrule
\end{tabular}
\caption{Mean and standard deviation (in subscript) of accuracy scores of classify-only models, and models proposed by \citet{pruthi2020weakly} and \citet{jain2020learning}, fined-tuned for sentiment analysis. Results highlighted in bold are significant with $p<0.05$. \label{tab:sentiment1}}
\end{table}


% \begin{table*}[t!]
% \centering
% \begin{tabular}{l c c c c}
% \toprule
% & \multicolumn{3}{c}{Dataset size}\\
% Evaluation Set &  $300$ & $600$ & $900$ & $1200$ \\
% \midrule
% % \multicolumn{5}{c}{SVM without/with rationales}\\
% % \midrule
% In-domain                                      
% & $77.0_{3.9}$/$77.6_{2.2}$
% & $78.5_{3.2}$/$82.3_{2.0}$
% & $80.5_{1.7}$/$\mathbf{84.9_{1.6}}$
% & $75.2_{3.5}$/$79.1_{3.4}$ \\

% CRD                                                               
% & $48.0_{2.9}$/$\mathbf{56.4_{1.3}}$
% & $48.3_{2.5}$/$\mathbf{58.0_{2.7}}$
% & $48.4_{2.3}$/$\mathbf{58.7_{1.8}}$
% & $48.3_{2.0}$/$\mathbf{58.2_{2.4}}$ \\ 

% SST-2                                                                                  
% & $52.2_{1.6}$/$\mathbf{62.9_{1.0}}$
% & $50.9_{3.0}$/$\mathbf{64.0_{0.9}}$
% & $51.3_{3.1}$/$\mathbf{64.9_{0.9}}$
% & $49.7_{0.3}$/$\mathbf{65.6_{1.5}}$\\

% Amazon                                             
% & $51.8_{1.5}$/$\mathbf{65.9_{1.9}}$
% & $52.4_{2.0}$/$\mathbf{66.5_{1.2}}$
% & $52.0_{2.9}$/$\mathbf{69.9_{0.4}}$
% & $50.9_{0.3}$/$\mathbf{68.7_{3.1}}$ \\ 

% Semeval                                                                                
% & $50.3_{1.4}$/$\mathbf{56.7_{1.1}}$
% & $50.3_{1.2}$/$\mathbf{56.4_{0.8}}$
% & $50.1_{0.5}$/$\mathbf{58.8_{1.3}}$
% & $49.8_{0.1}$/$\mathbf{58.0_{1.5}}$ \\

% Yelp                                                                                
% & $60.2_{4.0}$/$\mathbf{72.0_{2.4}}$
% & $57.3_{7.1}$/$\mathbf{74.5_{1.5}}$
% & $61.2_{4.6}$/$\mathbf{74.8_{2.5}}$
% & $55.7_{2.8}$/$\mathbf{74.8_{2.7}}$ \\
% % \midrule
% \bottomrule
% \end{tabular}
% \caption{ Mean and standard deviation (in subscript) of accuracy scores of classify-only SVM models (left) presented alongside accuracy scores of models trained with feature feedback (right), with increasing number of training-samples for sentiment analysis using the method proposed by \citet{zaidan2007using}. Results highlighted in bold show statistically significant difference with $p<0.05$.
% }
% \label{tab:sentiment3}
% \end{table*}


\begin{table}[t!]
\centering
\begin{tabular}{l c c}
\toprule
% & \multicolumn{3}{c}{Dataset size}\\
Test set & Classify-only & \citeauthor{zaidan2007using} \\
\midrule
% \multicolumn{5}{c}{SVM without/with rationales}\\
% \midrule
In-domain                                      
& $75.2_{3.5}$ & $79.1_{3.4}$ \\

CRD                                                               
& $48.3_{2.0}$ & $\mathbf{58.2_{2.4}}$ \\ 

SST-2
& $49.7_{0.3}$ & $\mathbf{65.6_{1.5}}$\\

Amazon
& $50.9_{0.3}$ & $\mathbf{68.7_{3.1}}$ \\ 

Semeval
& $49.8_{0.1}$ & $\mathbf{58.0_{1.5}}$ \\

Yelp
& $55.7_{2.8}$ & $\mathbf{74.8_{2.7}}$ \\
% \midrule
\bottomrule
\end{tabular}
\caption{ Mean and standard deviation (in subscript) of accuracy scores of classify-only SVM model versus SVM trained with feature feedback for sentiment analysis using \citet{zaidan2007using}'s method. Results highlighted in bold are significant with $p<0.05$.
}
\label{tab:sentiment3_only1200}
\vspace{-5mm}
\end{table}


% \begin{table}[t!]
% \centering
%     \small
% \begin{tabular}{l c c c}
% \toprule
% Test set &  Classify-only & \citeauthor{pruthi2020weakly}  & \citeauthor{jain2020learning}\\
% \midrule
% \multicolumn{4}{c}{BERT}\\
% \midrule
% In-domain & $88.7_{2.0}$ & $89.8_{0.8}$ & $77.7_{0.1}$\\
% RP & $62.9_{3.9}$ & $66.6_{0.6}$ & $57.9_{0.1}$\\
% RH & $76.9_{3.5}$ & $80.5_{1.9}$ & $70.7_{0.2}$\\
% MNLI-M & $69.7_{2.6}$ & $68.1_{1.9}$ & $69.8_{0.1}$\\
% MNLI-MM & $71.5_{2.7}$ & $69.2_{2.3}$ & $66.2_{0.1}$\\
% \midrule
% \multicolumn{4}{c}{ELECTRA}\\
% \midrule
% In-domain & $\mathbf{96.0_{0.2}}$ & $95.0_{0.3}$ & $85.4_{0.04}$\\
% RP & $80.8_{1.0}$ & $78.0_{0.6}$ & $72.2_{0.1}$\\
% RH & $88.9_{1.0}$ & $88.7_{0.9}$ & $79.7_{0.1}$\\
% MNLI-M & $86.5_{0.9}$ & $81.9_{2.1}$ & $77.1_{0.1}$\\
% MNLI-MM & $86.6_{0.8}$ & $82.1_{2.0}$ & $75.7_{0.1}$\\
% \bottomrule
% \end{tabular}
% \caption{Mean and standard deviation (in subscript) of F1 scores of models fine-tuned for NLI with increasing number of examples with feature feedback. Results highlighted in bold are significantly better than classify-only performance ($p<0.05$). \label{tab:sentiment1}}
% \vspace{-5mm}
% \end{table}
